Approaches to Asian Option Pricing with Discrete Dividends

The method and characteristics of several approaches to the pricing of discretely monitored arithmetic Asian options on stocks with discrete, absolute dividends are described. The contrast between method behaviors for options with an Asian tail and those with monitoring throughout their lifespan is emphasized. Rates of convergence are confirmed, but greater focus is put on actual performance in regions of accuracy which are realistic for use by practitioners. A hybrid approach combining Curran's analytical approximation with a two-dimensional finite difference method is examined with respect to the errors caused by the approximating assumptions. For Asian tails of equidistant monitoring dates, this method performs very well, but as the scenario deviates from the method's ideal conditions, the errors in the approximation grow unfeasible. For general monitoring straightforward solution of the full three-dimensional partial differential equation by finite differences is highly accurate but suffers from rapid degradation in performance as the monitoring interval increases. For options with long monitoring intervals a randomized quasi-Monte Carlo method with control variate variance reduction stands out as a powerful alternative.

==> tex/abstract/abstract.tex <==
\begin{abstract}
    \noindent The method and characteristics of several approaches to the
    pricing of discretely monitored arithmetic Asian options on stocks with
    discrete, absolute dividends are described. The contrast between method
    behaviors for options with an Asian tail and those with monitoring
    throughout their lifespan is emphasized. Rates of convergence are
    confirmed, but greater focus is put on actual performance in regions of
    accuracy which are realistic for use by practitioners. A hybrid approach
    combining Curran's analytical approximation with a two-dimensional finite
    difference method is examined with respect to the errors caused by the
    approximating assumptions.  For Asian tails of equidistant monitoring
    dates, this method performs very well, but as the scenario deviates from
    the method's ideal conditions, the errors in the approximation grow
    unfeasible. For general monitoring straightforward solution of the full
    three-dimensional partial differential equation by finite differences is
    highly accurate but suffers from rapid degradation in performance as the
    monitoring interval increases.  For options with long monitoring intervals
    a randomized quasi-Monte Carlo method with control variate variance
    reduction stands out as a powerful alternative.
\end{abstract}


==> tex/conclusion/conclusion.tex <==
Different approaches to the pricing of arithmetic Asian options with discrete,
absolute dividends were tested from the perspectives of convergence and
performance. It is clear that the best performance is obtained only with
knowledge of specifics regarding the target option. 

An option with an equidistant Asian tail benefits very little from the more
general approaches using Monte Carlo or solution of the full PDE. Irrespective
of dividend placement this case generally yields favorable results for the
approach combining Curran's approximation with finite difference extensions.
Introducing irregularity into the fixing placement is a more problematic issue,
and the improved accuracy of a finite difference method solving the full PDE
becomes potentially desirable without a catastrophic loss of performance.

Options with monitoring performed over a longer time period are more
problematic still, with the errors in Curran's approximation becoming highly
significant. Meanwhile, the cost of solving the full PDE grows dramatically,
and makes obtaining any reasonable degree of accuracy painful. While it could
be argued that the probabilistic nature of their convergence is undesirable,
Monte Carlo methods step up in these cases with their usual irreverence of
increases in dimensionality. Across a wide range of desired accuracies, then,
the approach of randomness (or quasi-randomness, as it were) makes a strong
argument for its existence.

Of further interest is the fact that the discussion thus far has neglected
another of the main strengths of Monte Carlo methods: its inherent parallelism.
While it is unlikely to carry the approach to superiority in the case of Asian
tails, it strengthens the argument that long monitoring intervals are the
domain of Monte Carlo.



==> tex/introduction/acknowledgements.tex <==
Jacob Lundgren would like to express gratitude to Uppsala
University's Professor Maciej Klimek for his guidance in the thesis project
upon which parts of this work is based. His suggestions on direction and focus
were highly valuable and were what allowed some of the more interesting results
to be obtained.

Yuri Shpolyanskiy would like to thank Jonas Hansbo, Itiviti's CSO and colleagues 
at Itiviti's Engineering: Dmitriy Ivanov, Dmitriy Kislin and Alexander Toropov 
for stimulating discussions.



==> tex/introduction/introduction.tex <==
The concept of an \emph{Asian} option payoff type consists in having the payoff
function depend on some notion of the \textbf{average} of the underlying
asset(s). The sense in which the average is understood, then, determines the
specific type of Asian option considered. While using geometric averages yields
convenient mathematics, arithmetic averages tend to be favored in practice
\citeCommand{curran-1994, dewynne-wilmott, zvan-main, haug-book, lord-2005}.

Another major distinction lies in the information upon which the average is
based --- the \emph{monitoring}. Options with continuous monitoring can be
studied as asymptotic cases, but options traded in actuality tend to instead
have a finite set of discrete \emph{monitoring dates} or \emph{fixings}. The
usual distinction between \emph{call} and \emph{put} variants applies without
modification. The strike price can either be \emph{fixed} or \emph{floating},
where the latter type utilizes the stock price at maturity as strike.

The Asian dependence on multiple samples of the underlying is often a highly
desirable characteristic in that it greatly reduces sensitivity to intentional
price manipulation. Further, if an actor is already exposed to the movement of
a particular asset over an interval of time, Asian options can assist in
accurately hedging this risk \citeCommand{zvan-main}.

Arithmetic Asian options are unwieldy constructs from a mathematical
perspective. In the case of discrete monitoring their payoff function involves
a sum of correlated log-normal variates, which is not possible to express as
any currently known distribution \citeCommand{curran-1994}. No methods of exact
analytical solution have thus yet been found, and resorting to approximations
or numerical methods are the only available alternatives. Among known
analytical approximations, Curran's approach \citeCommand{curran-1992} is believed to
be quite accurate as mentioned by Haug \citeCommand{haug-book}. Other approximations
can also be found in Haug's book. Lord in his paper \citeCommand{lord-2005} derives
analytical bounds for the value of arithmetic Asian options. As for the
standard numerical methods for option pricing, they are affected in varying
degrees by the additional complexity of the Asian payoff structure.

The exposition in this paper will revolve around the pricing of discretely
monitored, fixed strike arithmetic averaging Asian options with a single
underlying and general dividend structures. The placement of the monitoring
dates will remain briefly undefined, but particular focus will be on options
with monitoring solely as an \emph{Asian tail} --- a cluster of monitoring
dates in the vicinity of option maturity. Typical examples of such tails are
monitoring dates at each of the last 10 calendar or business days until (and
including) the maturity date. 

Allowing for general dividend structures --- in particular discrete dividends
paid by the underlying security --- is a complication that has not been handled
in the majority of previous expositions on related topics. Analytical
approximations cannot deal with discrete dividends. While mentioned and
theoretically handled in a few papers with numerical methods for Asian options
\citeCommand{dewynne-wilmott, zvan-main}, their results do not discuss the impact of
general dividends on convergence or performance characteristics. Ve\v{c}e\v{r}
considers discrete dividends, but his theory is applicable only to dividends
that are proportional to the underlying price, not predefined fixed dividend
amounts \citeCommand{vecer}. A significant part of the motivation for this paper is an
interest in the issues related to general discrete dividends and the resulting
effects on numerical solution methods. The practical goal is to reveal methods
that provide high computational performance both with and without discrete
dividends. Another desirable feature would be for the dividend correction to
have minimum possible impact on the surrounding algorithm, so as to simplify
both the implementation and the testing of result consistency.

\subsection{Numerical Complications}
For lattice methods, encountering fixings breaks the essential feature of
\emph{recombination}. Usually, the computational and memory complexity of
lattice methods is greatly alleviated by the Markov property of the value
process of many options. Introducing Asian monitoring dates voids this
property, and as a result nodes existing at a fixing will spawn individual
trees which in general will not reconnect. This explosion in state space
renders the method computationally unpalatable. It has been proposed
\citeCommand{lyuu-lattice} that discarding part of that space and recreating the lost
information through interpolation when required is a viable solution.

In largely similar fashion, modifying the Black-Scholes partial differential
equation (PDE) to account for the Asian payoff involves the introduction of an
additional spatial dimension \citeCommand{dewynne-wilmott, zvan-main}. As a result,
the finite difference method also suffers a severe, if generally less
explosive, increase in complexity. The standard grid structure is extended in
the averaging spatial dimension, creating a three-dimensional discrete problem
domain. In the case of discrete monitoring, the interaction of different levels
of the averaging dimension is isolated to the monitoring instants. Between
fixings the method can thus be interpreted as a set of independent finite
difference methods solving a discretization of the standard two-dimensional
Black-Scholes equation. The interaction is then implemented as jump conditions,
again with interpolation to reconstruct unavailable data as required. A few PDE
approaches \citeCommand{rogers-zhi, vecer} have also been suggested to avoid the
problem of increased dimensionality, and thus improve computational efficiency.
Unfortunately, these techniques cannot fully cover arbitrary discrete
dividends.

Among the strengths of the Monte Carlo method is its resilience to model
complications \citeCommand{joy-qmc}. Expecting it to be competitive with the more
rigid numerical methods for the examined options is thus not entirely baseless.
The method itself requires little adaptation to be able to valuate these
products, in essence only having each trajectory keep track of its running
average with respect to the fixing dates. The cost of this flexibility is a
comparatively unexciting rate of convergence which is also resistant to most
attempts at improvement. The implicit constant accompanying the rate of
convergence is a viable target, and many variance reduction techniques have
been developed for its minimization \citeCommand{glasserman-book}. One of the rare few
methods carrying the potential to affect the rate of convergence of Monte Carlo
estimators consists in replacing the random sampling in trajectory generation
with \emph{low-discrepancy sequences}. In reference to the alternative labeling
of such sequences as \emph{quasi-random}, the method is often termed
\emph{quasi-Monte Carlo}. All Monte Carlo methods can be extended in a
straightforward manner to account for discrete dividends, with only
insignificant growth of the computation time.

\subsection{Summary of Contributions}
This paper provides a high-level description of three approaches to the pricing
of arithmetic Asian options with general dividend structures. A finite
difference solver using the full PDE as described by Zvan et al.
\citeCommand{zvan-main} provides somewhat of a robust, na\"{i}ve solution to examine
the consistency of the other methods. A recent hybrid finite-difference approach 
\citeCommand{shpolyanskiy} combining the standard two-dimensional Black-Scholes PDE with 
Curran's analytical approximation \citeCommand{curran-1992} is outlined and
further augmented, providing a significantly faster approximative solution.
Finally, the Monte Carlo method offers a structurally simple alternative which
is also largely unaffected by model complications.

These approaches are studied from the perspectives of consistency, convergence
and computational complexity, yielding a characterization of when each one is
preferable. While the Curran-based approach can by its very nature not offer
consistency, it is found to quickly render highly accurate approximations in
situations fulfilling its assumptions. The explosion in computational
complexity of the full PDE method as the monitoring interval grows makes it a
weak candidate outside tail-type setups, despite strong convergence. The Monte
Carlo approach performs consistently irrespective of option characteristics,
and thus makes a strong argument for its use for options not covered by the
special cases of the other approaches.



==> tex/numerical-approaches/numerical-approaches.tex <==
\subsection{Full PDE Finite Differences}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=1.\textwidth]{full-pde}
    \caption{Structure of the full PDE FD solver}
    \label{fig:fd:full-pde}
\end{figure}
Introducing discrete Asian fixings into the Black-Scholes PDE expands the model
domain into an additional spatial dimension, representing the \emph{running
average} process \citeCommand{dewynne-wilmott, zvan-main}. Between monitoring dates,
the PDE remains unchanged as no information is exchanged between levels of the 
running average process. Meanwhile, an argument of absence of arbitrage implies 
that the option value just before a fixing must equal the one just after with an 
appropriately corrected running average level. This creates a jump condition that 
is applied at the fixing dates, and the resulting process is shown in Figure~\ref{fig:fd:full-pde}.

A similar condition is used for discrete dividends. Since a dividend is
necessarily accompanied by a drop in the value of the stock by the same amount,
absence of arbitrage again implies that the value of the option as a function
of the underlying stock must be shifted accordingly. Due to the structure of
finite difference grids, the values required to correct for the jump conditions
will in general not be available. Recreating approximations of this truncated
information can be done through interpolation, which in the following will be
four-point barycentric Lagrange interpolation \citeCommand{barycentric}.

The resulting PDE takes the form of the basic Black-Scholes PDE, with an
additional parameter for the running average process:
\begin{equation*}
    \partDeriv{V}{t} + \frac{1}{2} \sigma^{2}S^{2} \partDeriv{^{2}V}{S^{2}} 
    + (r - \delta) S \partDeriv{V}{S} - rV = 0, 
\end{equation*}
where $V(S, A, t)$ is the option price for stock value $S$ and the current arithmetic average 
$A$ accumulated over passed monitoring dates $t_{i} \leq t$ at time $t$, 
$\sigma$ is the volatility; $r$ is the interest rate; and $\delta$ is the dividend 
(convenience) yield. Prior to the first monitoring date $t_{1}$, $A$ is zero. 
The terminal condition at maturity $T$ is given by the payoff function $\Phi(S_{T}, A_{T})$: 
\begin{equation*}
    V(S_{T}, A_{T}, T) = \Phi(S_{T}, A_{T}).
\end{equation*}
These functions are specific to the type of contract: call or put, i.e.
\begin{equation*}
    \begin{aligned}
        \Phi_{call}(S_{T}, A_{T}) = \textrm{max}\left(A_{T} - K, 0\right), \\
        \Phi_{put}(S_{T}, A_{T}) = \textrm{max}\left(K - A_{T}, 0\right), 
    \end{aligned}
\end{equation*}
where $K$ is the strike price.

Letting $t_{-}$ denote the time an infinitesimally small time before the
$N^{\textrm{th}}$ fixing and $t_{+}$ the time an infinitesimally small time
after this fixing, the interaction between averaging levels is handled by the
jump condition
\begin{equation*}
    V\left(S, A_{t_{+}}, t_{+}\right) = V\left(S, \frac{(N - 1)A_{t_{-}} +
        S}{N}, t_{-}\right),
\end{equation*}
and letting the same notation instead denote the surroundings of a discrete
dividend of size $D$, the second jump condition is
\begin{equation*}
    V\left(S_{t_{+}}, A, t_{+}\right) = V\left(S_{t_{-}} + D, A, t_{-}\right).
\end{equation*}

\subsection{Hybrid Curran-Finite Differences}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=1.\textwidth]{shpolyanskiy}
    \caption{Structure of the Curran-based FD solver}
    \label{fig:fd:shpolyanskiy}
\end{figure}
An approach has previously been described \citeCommand{shpolyanskiy} for efficiently
estimating the value of Asian options where any discrete dividend payments are
performed prior to the first monitoring date. At its core is an approximation
suggested by Curran \citeCommand{curran-1992}, which introduces a conditioning on the
geometric average to obtain an estimation of the value of an arithmetic Asian
option on a stock not paying discrete dividends. It is possible to allow for
such dividends before the first monitoring date, by setting up a standard
Black-Scholes PDE with maturity at the last dividend payment. The approximation is then
used to generate the terminal condition, and a finite difference method can be
used to solve for the values at current time. The solution flow is illustrated
in Figure~\ref{fig:fd:shpolyanskiy}, with $t_{D^{-}}$ denoting the final
dividend payment.

An additional approximation allows for absolute-valued discrete dividends
inside the monitoring interval. Assuming that the dividends are small in
comparison to the strike, their impact can be transferred to the strike price.
Let $D$ be an absolute-valued discrete dividend payment due at a time $t_{D^{+}}$
which is inside the monitoring interval. Denote by $t_{1}, t_{2}, \ldots,
t_{N}$ the times of the fixings. Let further $N$ denote the total amount of
monitoring dates, and $n_{\textrm{aff}}$ the first fixing following --- and
thus affected by --- the dividend. With the constant interest rate $r$ and
dividend yield $\delta$, the dividend effect can be compensated for by
increasing the strike price by
\begin{equation*}
    K_{\textrm{shift}} = \frac{D}{N}\sum_{i=n_{\textrm{aff}}}^{N}e^{(r -
        \delta)(t_{i} - t_{D^{+}})},
\end{equation*}
i.e.\ the amount by which the compounded dividend would have reduced the 
final arithmetic average $A_{T}$ via drops in spot price at future
fixings. This ignores the effect of the dividend on the stock process dynamics,
which introduces an error. The size of this error is one of the factors
examined in the following. When dividends are present in the monitoring
interval, the initialization using Curran's approximation is done at the time
of the first fixing, and the finite difference solver proceeds from this point.

\subsection{Monte Carlo}
\begin{figure}[ht!]
    \includegraphics[width=0.9\textwidth]{monte-carlo}
    \caption{Structure of the Monte Carlo solver}
    \label{fig:mc:mc}
\end{figure}
In the case of Monte Carlo methods, the tracking of the averaging dimension is
significantly less taxing. Each trajectory keeps a running average value which
is updated when fixing dates are hit as shown in Figure~\ref{fig:mc:mc}, but no
new dependency structures are introduced. As a result, neither the overall
complexity nor the inherent parallelism of the method are affected to any
considerable degree. The disappointing convergence characteristics of the
approach remain an issue, however --- the price of simplicity and adaptability
to complications.

In order to reduce the variance of the Monte Carlo estimator, a wide variety of
\emph{variance reduction techniques} have been developed
\citeCommand{glasserman-book}. While they are unable to affect the overall behavior
and rate of the convergence, their use is intended to result in lower absolute
variances for any given setup.

The method of \emph{antithetic variates} consists in inverting the samples
utilized to generate each trajectory and produce what is essentially a mirror
image. This ensures that all scenarios of improbably high stock growth are
accompanied by an equivalently low counterpart and vice versa. For options
where the mapping from underlying trajectory to option value is monotone, this
reduces the variance of the overall estimator.

\emph{Control variate} methods are formalizations of the idea that knowledge of
processes correlated with the option value process can be used to improve
estimations of the latter. Assume that there is a process correlated with the
option value process, which can be evaluated using the same underlying
trajectories, and has a known expectation. This process can then be used as a
control in simulations of the option value. For each trajectory, the difference
between the estimate of the control process and its known expectation is used
to correct the estimator of the correlated option value process.

It remains to find candidates for control processes. In the case of arithmetic
Asian options, the closely related but mathematically more convenient geometric
Asian options have been suggested. The value of these options is analytically
known for underlyings with up to a continuous dividend yield, but since the
target is to allow for general dividend structures the control is not directly
usable. What is attempted is instead to simulate pairs of trajectories using
the same normal samples, with one being uncorrected for discrete dividends. A
geometric Asian option on the underlying without discrete dividends is then
used as a control, with the assumption that the positive correlation should
remain largely unaffected.

Variance reduction techniques are potent tools for reducing the implicit
constant in the variance of the Monte Carlo estimator. The more problematic
issue of the order $0.5$ of convergence in number of trajectories, however,
generally remains unaffected. A technique with the potential to improve
performance in both regards, however, consists in steering the random sampling
to distribute points in an artificially even manner. This can be done by the
use of \emph{low-discrepancy sequences} to feed the simulation, instead of the
more common pseudo-random number generators.

Low-discrepancy (or \emph{quasi-random}) sequences are \textbf{deterministic}
constructs that derive their name from the concept of \emph{discrepancy}, which
informally can be described as a measure of how ``unevenly'' a set of points is
distributed in a domain.  Equivalently, the discrepancy can be interpreted as
the amount of \emph{clustering} the set of points exhibits. Each point added to
a low-discrepancy sequence is placed to minimize the discrepancy of the
resulting set of points, thus ensuring that the placement is in some sense
``optimal'' irrespective of the number of points used.

A wide variety of low-discrepancy sequences are available, with differing
characteristics. A commonly used type is the Sobol' sequence, the generation of
which is readily expressed as a highly efficient computational algorithm. The
algorithm requires exogenous information both for its initialization and
generation processes, and the choices affect how well the resulting sequence
optimizes measures of discrepancy. This selection is anything but trivial, but
authors Joe and Kuo \citeCommand{joe-kuo-2003, joe-kuo-2008} have graciously made the
results of their research on the matter available for public use.

To obtain samples of the normal distribution, coordinates of the points of a
low-discrepancy sequence are fed into a distribution conversion algorithm such
as straightforward inversion of the normal cumulative distribution function or
the Box-Muller algorithm. There is debate \citeCommand{goncu-mc, joy-qmc} as to
whether the latter alternative has an undesirable impact on the distributive
properties of low-discrepancy sequences. In the interest of retaining focus,
the Box-Muller algorithm is used in the following for reasons of computational
efficiency.

One of the advantages of standard Monte Carlo methods is the fact that the
error in the estimator is asymptotically normal, allowing for estimation of the
error itself by repeated invocation. With the deterministic sampling of
standard quasi-Monte Carlo, however, this is not an option. In order to regain
this ability, randomness can be partially reintroduced into the quasi-Monte
Carlo algorithm, resulting in what is commonly termed \emph{randomized
quasi-Monte Carlo (RQMC)}. This randomization can be done in a multitude of
ways, with varying computational and implementational complexity and also with
different effects on the discrepancy of the resulting sequence.

One way of performing such a randomization is that of using a \emph{random
shift}. A vector of the same dimensionality as the quasi-random points is
filled with uniform variates on $[0, 1)$, and added elementwise to each point
in the sequence, keeping only the fractional part. It is important to note, 
however, that this procedure does \textbf{not} fully preserve all desirable
distributional properties of the low-discrepancy sequence
\citeCommand{randomized-quasi}.

\subsection{Implementation Details}
The experiments detailed in the following use sequential implementations
written in C++. All finite difference implementations utilize the
Crank-Nicolson scheme \citeCommand{crank-nicolson} as their main method of
solution. The interaction of this scheme with the class $C^{0}$ terminal
condition and jump conditions is, however, known to result in impaired
convergence rates \citeCommand{rannacher, unsmooth-solution}. To rectify this,
the suggested solution of splitting the first step into four steps of the
implicit Euler scheme is used.  This technique is known as Rannacher time
stepping, and is applied at the start of each interval of continuity. In other
words at maturity, dividend dates and --- in the case of the full PDE method
--- at fixing dates.

The algorithm used for the Monte Carlo time stepping is direct solution of the
underlying dynamics of the geometric Brownian motion driving the stock process,
i.e.
\begin{equation*}
    S_{t_{i+1}} = S_{t_{i}}\exp\left[\left(r - \delta\right)\left(t_{i+1} -
        t_{i}\right) + \sigma \sqrt{t_{i+1} - t_{i}} Z\right],
\end{equation*}
where $t_{i}$ and $t_{i+1}$ are two consecutive time points and $Z \sim
\mathcal{N}(0, 1)$. The ability in the standard Black-Scholes framework to
perform exact stepping of this type means that taking extraneous steps shows no
improvement in accuracy. The Monte Carlo methods thus step only onto dividends
and fixings, with no intermediate steps.

For both the full PDE finite difference method and the Monte Carlo methods, the
correction order of perfectly overlapping fixings and dividends must be
defined. In a chronological sense, the used implementations apply dividend
payouts before Asian monitoring, while the reverse-flowing finite difference
method inverts this to obtain consistent results.

The implementation of Curran's approximation is based on the description by
Haug \citeCommand{haug-book}, and assumes equidistant monitoring data. The impact of
this approximation for non-equidistant fixing placements is one of the issues
investigated in the following. The functionality for discrete dividends inside
the monitoring interval also only allows compounding from the fixing following
the dividend date, a fact which is assumed to generally have a significantly
smaller impact.



==> tex/results-discussion/results-discussion.tex <==
\subsection{Testing Setup}
\newcommand{\setupstyle}[1]{\emph{#1}}
%\begin{figure}
%    \centering
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{full-asian-no-div}
%        \caption{\setupstyle{full-none-eq}}
%    \end{subfigure}%
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{full-asian-no-div-non-equidistant}
%        \caption{\setupstyle{full-none-neq}}
%    \end{subfigure}
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{full-asian-div-inside}
%        \caption{\setupstyle{full-late-eq}}
%    \end{subfigure}%
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{full-asian-div-inside-non-equidistant}
%        \caption{\setupstyle{full-late-neq}}
%    \end{subfigure}
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{asian-tail-no-div}
%        \caption{\setupstyle{tail-none-eq}}
%    \end{subfigure}%
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{asian-tail-no-div-two-weekends}
%        \caption{\setupstyle{tail-none-neq}}
%    \end{subfigure}
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{asian-tail-div-outside}
%        \caption{\setupstyle{tail-early-eq}}
%    \end{subfigure}%
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{asian-tail-div-outside-two-weekends}
%        \caption{\setupstyle{tail-early-neq}}
%    \end{subfigure}
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{asian-tail-div-inside}
%        \caption{\setupstyle{tail-late-eq}}
%    \end{subfigure}%
%    \begin{subfigure}{.5\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{asian-tail-div-inside-two-weekends}
%        \caption{\setupstyle{tail-late-neq}}
%    \end{subfigure}%
%    \caption{Test setups}
%    \label{fig:tests:setups}
%\end{figure}

\begin{table}[ht!]
    \centering
    \scalebox{0.8}{%
    \cfinput{tables/monitoring_setups.tex}
    }
    \caption{Discrete monitoring times for the monitoring setups}
    \label{tab:tests:monitoring-setups}
\end{table}
\begin{table}[ht!]
    \centering
    \scalebox{0.8}{%
    \cfinput{tables/dividend_setups.tex}
    }
    \caption{Times and sizes of discrete dividend payments for the dividend
    setups}
    \label{tab:tests:dividend-setups}
\end{table}
In order to understand the characteristics of the solvers, a set of varying
option setups is used. The situations will in the following be labeled
according to the scheme

\centerline{\setupstyle{$<$tail/full$>$}-\setupstyle{$<$none/early/late$>$}-\setupstyle{$<$eq/neq$>$,}}

\noindent where the fields carry the following meaning:
\begin{itemize}
    \item \setupstyle{$<$tail/full$>$} --- Option fixings arranged in an Asian tail
        or throughout the option lifespan
    \item \setupstyle{$<$none/early/late$>$} --- Dividend placement and existence
    \item \setupstyle{$<$eq/neq$>$} --- Fixings equidistant or non-equidistant.
\end{itemize}
The setup details are shown in Tables~\ref{tab:tests:monitoring-setups}
and~\ref{tab:tests:dividend-setups}, outlining respectively the monitoring
times and the dividend times with associated sizes. The \setupstyle{tail-eq}
scenarios use the last $10$ calendar days for monitoring, while the
\setupstyle{tail-neq} scenarios use the last $10$ business days with two
weekends contained within the monitoring interval. There is no particular
rationale to the selection of the \setupstyle{full-neq} monitoring dates,
except that the number of fixings before and after each dividend in the
\setupstyle{late} dividend setup is consistent with the equidistant case.


The following parameters are used throughout
\begin{itemize}
    \item Interest rate: $5\%$ annually
    \item Dividend yield: $2\%$ annually
    \item Volatility: $40\%$ annually
    \item Maturity: $1$ year
    \item Payoff and exercise: European Asian call
    \item Strike price: $100$ arb.\ units.
\end{itemize}
The discrete dividends are fully absolute valued with the values (in arb.\
units) $[2.1$, $1.9$, $2.051$, $1.949]$.

Since the full PDE finite difference method consists only of standard numerical
techniques applied to the original mathematical problem, its result on a
$10^{4} \times 10^{4} \times 10^{4}$ grid is used as a reference for all error
measurements. As a result, \textbf{the errors given for the full PDE method are
self-referential}. Arguing for the correctness of its use as a reference thus
requires the corroboration of the Monte Carlo methods converging to the same
value, and the discussion must be viewed from a holistic standpoint to be
considered accurate.

Stated errors for the finite difference-based solvers are given in terms of
fraction of the reference value, and ignore polarity of error. The given values
are the maximum relative errors in the stock interval $[0.6K, 1.4K]$, where $K$
is the strike price. For the Monte Carlo methods, only the value for stock
price equal to strike price is considered, and standard deviations of the
estimator are given as measures of error. \textbf{Direct comparison between the
finite difference solvers and Monte Carlo solvers is thus not possible without
judgment calls regarding the conversion rate between deterministic error and
probabilistic deviation}.

\begin{table}[ht!]
    \centering
    \scalebox{0.8}{%
    \cfinput{tables/stddev_confidence.tex}
    }
    \caption{Probability of errors being within multiples of standard
        deviations}
    \label{tab:tests:stddev-confidence}
\end{table}
The correspondences between number $n$ of standard deviations $\sigma_{std}$ and the
probability $P$ with which the error is within $(-n\sigma_{std}, n\sigma_{std})$ as given
in Table~\ref{tab:tests:stddev-confidence} can be useful in deciding on desired
size of standard deviation. The standard deviations are generated from sampling
the Monte Carlo estimator $10^{3}$ times, and are shown relative to the
reference value provided by the full PDE finite difference solver. The
expression for the shown relative standard deviation is thus
\begin{equation*}
    \sigma_{std, rel} = \frac{1}{V_{ref}}\sigma_{std} = \frac{1}{V_{ref}}
    \sqrt{\frac{\sum_{i=1}^{10^{3}}(V_{i, MC} - V_{ref})^{2}}{10^{3} - 1}},
\end{equation*}
where $V_{ref}$ is the reference value and $V_{i, MC}$, $i \in [1, 10^{3}]$ are
independent samples from the Monte Carlo estimator. The subtraction of $1$ in
the denominator is due to Bessel's correction \citeCommand{bessel-correction} for bias
in sample variance estimators.

\subsection{Convergence Characteristics}
\begin{figure}
    \centering
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{full-pde-div-outside-node-conv}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{full-pde-div-outside-avg-conv}
    \end{subfigure}
    \vspace{0.4cm}
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=.5\linewidth]{full-pde-div-outside-time-conv}
    \end{subfigure}
    \caption{Orders of convergence for the full PDE FD method
        \setupstyle{(tail-early-eq)}}
    \label{fig:tests:full-pde-conv}
\end{figure}
The convergence in all three dimensions of the full PDE finite difference
solver is of second order as displayed in Figure~\ref{fig:tests:full-pde-conv}
for \setupstyle{tail-early-eq}. The dimensions not under examination are fixed
at $10^{4}$ nodes to isolate the error from each dimension. From the
perspective of convergence, this behavior is consistent throughout all tested
scenarios, with only the implicit constant changing. Using the heuristic that
refinement should be in the dimension of greatest error, these plots also
suggest the ratio $4:2:1$ for stock:average:time nodes for this scenario. This
ratio remains reasonably constant between scenarios with similar monitoring
intervals (introducing a dividend shifts it slightly to $10:6:3$). For options
with monitoring throughout their lifespan, the ratio $10:3:3$ can be found in
similar fashion.

\begin{figure}
    \centering
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{shpolyanskiy-div-outside-node-conv}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{shpolyanskiy-div-outside-time-conv}
    \end{subfigure}%
    \caption{Orders of convergence for the Curran-based FD solver
        \setupstyle{(tail-early-eq)}}
    \label{fig:tests:shpolyanskiy-conv}
\end{figure}
Figure~\ref{fig:tests:shpolyanskiy-conv} shows the convergence behavior of the
Curran-based solution method for \setupstyle{tail-early-eq} --- a case which
interacts well with the assumptions of the approximations. The error in each
dimension is isolated as above. Again, second order convergence in all
dimensions is observed, until the point where the difference in converged
values between the approximation and the full PDE solution becomes dominant.
Due to the approximations involved, this difference is highly dependent on the
considered situation, and much of the exposition in the following will be
examining how the approximations fare in the different option scenarios.

\begin{figure}
    \centering
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{mc-method-comp}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{mc-method-perf}
    \end{subfigure}%
    \caption{Convergence, performance for the Monte Carlo variants
        \setupstyle{(tail-early-eq)}}
    \label{fig:tests:mc-method-comp}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{mc-rqmc-vs-control}
    \caption{Behavior of standard vs controlled RQMC
        \setupstyle{(tail-late-neq)}}
    \label{fig:tests:mc-rqmc-vs-control}
\end{figure}
For the Monte Carlo variants, the first consideration is which type to use.
Figure~\ref{fig:tests:mc-method-comp} shows the convergence and performance
behaviors for \setupstyle{tail-early-eq} of the following Monte Carlo
configurations
\begin{itemize}
    \item Standard Monte Carlo without variance reduction
    \item Standard Monte Carlo with antithetic variates and control variates
    \item Randomized quasi-Monte Carlo without variance reduction
    \item Randomized quasi-Monte Carlo with control variates.
\end{itemize}
The observed result --- the control variate RQMC method exhibiting superior
behavior almost without exception --- is found consistently throughout testing.
Results for the Monte Carlo approach will thus be generated using this method.

It should be mentioned that the rate of convergence of the basic RQMC method is
slightly greater than that of the control variate-corrected RQMC method. The
error of the standard RQMC solver is $\mathcal{O}(N^{-0.79})$, while that of
the controlled RQMC solver is $\mathcal{O}(N^{-0.63})$ --- both of which are
within the range of capacity of QMC \citeCommand{glasserman-book}. Accordingly,
despite the substantially smaller constant term for the control variate
version, for sufficiently large numbers of trajectories it is overtaken performance-wise by the
standard RQMC solver as shown in Figure~\ref{fig:tests:mc-rqmc-vs-control}.
This figure also helps substantiate the claims to correctness and high accuracy
of both the full PDE finite difference method used as a reference and the Monte
Carlo methods themselves.

\subsection{Error from Approximations}
\begin{table}[ht!]
    \centering
    \scalebox{0.8}{%
    \cfinput{tables/curran_no_div_err.tex}
    }
    \caption{Curran approximation errors and time consumption}
    \label{tab:tests:curran-no-div-err}
\end{table}
\begin{table}[ht!]
    \centering
    \scalebox{0.8}{%
    \cfinput{tables/curran_div_err.tex}
    }
    \caption{Curran-based FD solver errors and time consumption}
    \label{tab:tests:curran-div-err}
\end{table}

Understanding the impact of the approximations involved in the Curran-based
solver is imperative in determining its usefulness. Two categories of scenarios
are treated separately --- those with discrete dividends and those without. For
the scenarios without discrete dividends, the Curran approximation can be used
without modification, yielding the errors shown in
Table~\ref{tab:tests:curran-no-div-err}. The scenarios containing discrete
dividends, however, require the finite difference extensions previously
outlined. Error bounds for these cases, as well as the time required to reach
them, are shown in Table~\ref{tab:tests:curran-div-err}. As shown by the case
\setupstyle{tail-late-eq}, the described correction for dividends inside the
monitoring interval renders accurate results when the monitoring period is
short, and the effects of the dividend on the stock dynamics thus are limited.

While the question of what is acceptable accuracy is highly dependent on
application, it seems difficult to ignore the percent-magnitude errors incurred
by Curran's approximation for Asian options with fixings distributed throughout
their lifespan. Inversely, only those with highly specialized requirements (and
great faith in the model) should be unsatisfied by the numbers posted for the
scenarios with equidistant fixings in an Asian tail. The areas where judgment
calls will be more diverse are the borderlands consisting of non-equidistant
fixings in an Asian tail formation, as accuracy takes a very real hit from such
fixing layouts.

\subsection{Performance}
\begin{figure}
    \centering
    \includegraphics[scale=0.9]{full-pde-comp-perf}
    \caption{Effects of monitoring interval on full PDE solver performance}
    \label{fig:tests:full-pde-comp-perf}
\end{figure}
From a performance and accuracy standpoint, the full PDE finite difference
solver is generally unconcerned about the specifics of dividend and fixing
placement and sizes, but the particular issue of monitoring interval size has
an immense impact on the execution time.
Figure~\ref{fig:tests:full-pde-comp-perf} displays the difference in execution
time required to reach different degrees of accuracy for an Asian tail case and
a full Asian case. Due to the fact that the averaging dimension collapses to a
single level $A=0$ outside monitoring intervals, the full PDE method is significantly
more palatable in scenarios with short such intervals.

There is an important caveat regarding the data displayed in
Figure~\ref{fig:tests:full-pde-comp-perf} which is related to the error
estimation. The error shown is the worst case scenario, i.e.\ the sum of the
largest estimated errors in each dimension for the setup. The choice of run
parameters for the next datapoint is done by refining the dimension for which
the estimated error is currently the largest.

\begin{figure}
    \centering
    \includegraphics[scale=0.9]{mc-comp-perf}
    \caption{Effects of monitoring interval on MC solver performance}
    \label{fig:tests:mc-comp-perf}
\end{figure}
In contrast to the full PDE FD solver, the Monte Carlo solvers are affected
comparatively little by changing the monitoring interval, as
Figure~\ref{fig:tests:mc-comp-perf} shows.
Figures~\ref{fig:tests:full-pde-comp-perf} and~\ref{fig:tests:mc-comp-perf} are
highly useful in establishing regions of usefulness for the different methods.
Due to the different measures of error, rigorous comparative statements are
again impossible. Irrespective of the conversion mapping between the errors,
however, it would not seem unreasonable to say that the Monte Carlo methods are
at least competitive --- if not superior --- for options with monitoring dates
throughout their lifespan. It is also clear that the Monte Carlo methods have a
significant amount of ground to make up through their inherent parallelism to
be considered a contender for Asian tail scenarios.



==> tex/results-discussion/tables/curran_div_err.tex <==
\begin{tabular}{| c || c | c | c | c | c | c |}
    \hline
    Scenario & \setupstyle{tail-early-eq} & \setupstyle{tail-early-neq} &
        \setupstyle{tail-late-eq} & \setupstyle{tail-late-neq} &
        \setupstyle{full-late-eq} & \setupstyle{full-late-neq} \\ \hline
    Rel.\ Error & 1.7e-6 & 3.3e-3 & 6.1e-5 & 3.2e-3 & 9.5e-2 & 2.6e-2
        \\ \hline
    Time ($\mu$s) & 9.3e3 & 4.6e2 & 1.3e4 & 4.1e2 & 8.5e1 &
        2.4e2 \\
    \hline
\end{tabular}



==> tex/results-discussion/tables/curran_no_div_err.tex <==
\begin{tabular}{| c || c | c | c | c |}
    \hline
    Scenario & \setupstyle{tail-none-eq} & \setupstyle{tail-none-neq} &
        \setupstyle{full-none-eq} & \setupstyle{full-none-neq} \\ \hline
    Rel.\ Error & 5.1e-6 & 2.9e-3 & 1.1e-2 & 1.1e-1 \\ \hline
    Time ($\mu$s) & 5.8e-1 & 5.8e-1 & 6.7e-1 & 6.7e-1 \\
    \hline
\end{tabular}



==> tex/results-discussion/tables/dividend_setups.tex <==
\scalebox{0.8}{%
    \begin{tabular}{| c || c | c | c | c |}
        \hline
        \setupstyle{early} & 0.0548 & 0.3048 & 0.5548 & 0.8048 \\ \hline
        \setupstyle{late} & 0.2390 & 0.4890 & 0.7390 & 0.9890 \\ \hline
        Size & 2.1 & 1.9 & 2.051 & 1.949 \\
        \hline
    \end{tabular}
}



==> tex/results-discussion/tables/monitoring_setups.tex <==
\begin{tabular}{| c || c | c | c | c | c | c | c | c | c | c |}
    \hline
    \setupstyle{tail-eq} & 0.9753 & 0.9781 & 0.9808 & 0.9836 & 0.9863 &
        0.9890 & 0.9918 & 0.9945 & 0.9973 & 1 \\ \hline
    \setupstyle{tail-neq} & 0.9644 & 0.9671 & 0.9699 & 0.9726 & 0.9808
        & 0.9836 & 0.9863 & 0.9890 & 0.9918 & 1  \\ \hline
    \setupstyle{full-eq} & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 &
        0.8 & 0.9 & 1 \\ \hline
    \setupstyle{full-neq} & 0.114 & 0.203 & 0.295 & 0.445 & 0.551 & 0.692 &
        0.710 & 0.778 & 0.932 & 1 \\
    \hline
\end{tabular}



==> tex/results-discussion/tables/stddev_confidence.tex <==
\begin{tabular}{| c || c | c | c | c |}
    \hline
    n & 1 & 2 & 3 & 4 \\ \hline
    P & 0.682689 & 0.954500 & 0.997300 & 0.999937 \\
    \hline
\end{tabular}


